Goals as Reward-Producing Programs

People are remarkably capable of generating their own goals, beginning with child's play and continuing into adulthood. Despite considerable empirical and computational work on goals and goal-oriented behavior, models are still far from capturing the richness of everyday human goals. Here, we bridge this gap by collecting a dataset of human-generated playful goals (in the form of scorable, single-player games), modeling them as reward-producing programs, and generating novel human-like goals through program synthesis. Reward-producing programs capture the rich semantics of goals through symbolic operations that compose, add temporal constraints, and allow for program execution on behavioral traces to evaluate progress. To build a generative model of goals, we learn a fitness function over the infinite set of possible goal programs and sample novel goals with a quality-diversity algorithm. Human evaluators found that model-generated goals, when sampled from partitions of program space occupied by human examples, were indistinguishable from human-created games. We also discovered that our model's internal fitness scores predict games that are evaluated as more fun to play and more human-like.

==> PCFG.tex <==
\lstset{columns=fullflexible,
        basicstyle=\tiny,
        mathescape=true,
        sensitive=true,
        literate=
               {>}{$\rightarrow{}$}{1}
               {==}{$={}$}{1},
        morekeywords={game,:setup,:constraints,:terminal,:scoring,once-measure},
        morecomment={[l][\color{CommentGreen}]{\#\#}},
        keywords=[2]{building_size,distance,distance_side,x_position},
        keywordstyle=[2]\color{red},
        keywords=[3]{above,adjacent,adjacent_side,agent_crouches,agent_holds,
                     between,broken,equal_x_position,equal_z_position,
                     faces,game_over,game_start,in,in_motion,is_setup_object,
                     object_orientation,on,open,opposite,rug_color_under,same_color,
                     same_object,same_type,toggled_on,touch},
        keywordstyle=[3]\color{orange},
        keywords=[4]{total-time,total-score},
        keywordstyle=[4]\color{purple},
        }

\begin{lstlisting}
START > (define GAME_DEF DOMAIN_DEF SETUP_DEF CONSTRAINTS_DEF TERMINAL_DEF SCORING_DEF )    (P = 1.0000)
GAME_DEF > (game ID )    (P = 1.0000)

ID > /[a-z0-9][a-z0-9\-]+/    (P = 1.0000)

DOMAIN_DEF > (:domain ID )    (P = 1.0000)

SETUP_DEF > (:setup SETUP )    (P = 1.0000)

SETUP > SETUP_AND    (P = 0.2322)

SETUP > SETUP_OR    (P = 0.0372)

SETUP > SETUP_NOT    (P = 0.0372)

SETUP > SETUP_EXISTS    (P = 0.2074)

SETUP > SETUP_FORALL    (P = 0.1455)

SETUP > SETUP_STATEMENT    (P = 0.3406)

SETUP_AND > (and [ SETUP ]+ )    (P = 1.0000)

SETUP_OR > (or [ SETUP ]+ )    (P = 1.0000)

SETUP_NOT > (not SETUP )    (P = 1.0000)

SETUP_EXISTS > (exists VARIABLE_LIST SETUP )    (P = 1.0000)

VARIABLE_LIST > ( VARIABLE_TYPE_DEF )    (P = 0.9252)

VARIABLE_LIST > ( COLOR_VARIABLE_TYPE_DEF )    (P = 0.0340)

VARIABLE_LIST > ( ORIENTATION_VARIABLE_TYPE_DEF )    (P = 0.0204)

VARIABLE_LIST > ( SIDE_VARIABLE_TYPE_DEF )    (P = 0.0204)

VARIABLE_TYPE_DEF > [ VARIABLE ]+ - TYPE_DEFINITION    (P = 1.0000)

VARIABLE > /\?[a-w][a-z0-9]*/    (P = 1.0000)

TYPE_DEFINITION > OBJECT_TYPE    (P = 0.8687)

TYPE_DEFINITION > EITHER_TYPES    (P = 0.1313)

OBJECT_TYPE > NAME    (P = 1.0000)

NAME > /[A-Za-z][A-Za-z0-9_]*/    (P = 1.0000)

EITHER_TYPES > (either [ OBJECT_TYPE ]+ )    (P = 1.0000)

COLOR_VARIABLE_TYPE_DEF > [ COLOR_VARIABLE ]+ - COLOR_TYPE_DEFINITION    (P = 1.0000)

COLOR_VARIABLE > /\?x[0-9]*/    (P = 1.0000)

COLOR_TYPE_DEFINITION > COLOR_TYPE    (P = 0.5625)

COLOR_TYPE_DEFINITION > EITHER_COLOR_TYPES    (P = 0.4375)

COLOR_TYPE > COLOR    (P = 1.0000)

COLOR > BLUE    (P = 0.0909)

COLOR > BROWN    (P = 0.0909)

COLOR > GRAY    (P = 0.0909)

COLOR > GREEN    (P = 0.0909)

COLOR > ORANGE    (P = 0.0909)

COLOR > PINK    (P = 0.0909)

COLOR > PURPLE    (P = 0.0909)

COLOR > RED    (P = 0.0909)

COLOR > TAN    (P = 0.0909)

COLOR > WHITE    (P = 0.0909)

COLOR > YELLOW    (P = 0.0909)

EITHER_COLOR_TYPES > (either [ COLOR ]+ )    (P = 1.0000)

ORIENTATION_VARIABLE_TYPE_DEF > [ ORIENTATION_VARIABLE ]+ - ORIENTATION_TYPE_DEFINITION    (P = 1.0000)

ORIENTATION_VARIABLE > /\?y[0-9]*/    (P = 1.0000)

ORIENTATION_TYPE_DEFINITION > ORIENTATION_TYPE    (P = 0.5000)

ORIENTATION_TYPE_DEFINITION > EITHER_ORIENTATION_TYPES    (P = 0.5000)

ORIENTATION_TYPE > ORIENTATION    (P = 1.0000)

ORIENTATION > DIAGONAL    (P = 0.2500)

ORIENTATION > SIDEWAYS    (P = 0.2500)

ORIENTATION > UPRIGHT    (P = 0.2500)

ORIENTATION > UPSIDE_DOWN    (P = 0.2500)

EITHER_ORIENTATION_TYPES > (either [ ORIENTATION ]+ )    (P = 1.0000)

SIDE_VARIABLE_TYPE_DEF > [ SIDE_VARIABLE ]+ - SIDE_TYPE_DEFINITION    (P = 1.0000)

SIDE_VARIABLE > /\?z[0-9]*/    (P = 1.0000)

SIDE_TYPE_DEFINITION > SIDE_TYPE    (P = 0.5000)

SIDE_TYPE_DEFINITION > EITHER_SIDE_TYPES    (P = 0.5000)

SIDE_TYPE > SIDE    (P = 1.0000)

SIDE > BACK    (P = 0.2500)

SIDE > FRONT    (P = 0.2500)

SIDE > LEFT    (P = 0.2500)

SIDE > RIGHT    (P = 0.2500)

EITHER_SIDE_TYPES > (either [ SIDE ]+ )    (P = 1.0000)

SETUP_FORALL > (forall VARIABLE_LIST SETUP )    (P = 1.0000)

SETUP_STATEMENT > SETUP_GAME_CONSERVED    (P = 0.6230)

SETUP_STATEMENT > SETUP_GAME_OPTIONAL    (P = 0.3770)

SETUP_GAME_CONSERVED > (game-conserved SUPER_PREDICATE )    (P = 1.0000)

SUPER_PREDICATE > SUPER_PREDICATE_AND    (P = 0.1914)

SUPER_PREDICATE > SUPER_PREDICATE_OR    (P = 0.0200)

SUPER_PREDICATE > SUPER_PREDICATE_NOT    (P = 0.1780)

SUPER_PREDICATE > SUPER_PREDICATE_EXISTS    (P = 0.0252)

SUPER_PREDICATE > SUPER_PREDICATE_FORALL    (P = 0.0100)

SUPER_PREDICATE > FUNCTION_COMPARISON    (P = 0.0490)

SUPER_PREDICATE > PREDICATE    (P = 0.5265)

SUPER_PREDICATE_AND > (and [ SUPER_PREDICATE ]+ )    (P = 1.0000)

SUPER_PREDICATE_OR > (or [ SUPER_PREDICATE ]+ )    (P = 1.0000)

SUPER_PREDICATE_NOT > (not SUPER_PREDICATE )    (P = 1.0000)

SUPER_PREDICATE_EXISTS > (exists VARIABLE_LIST SUPER_PREDICATE )    (P = 1.0000)

SUPER_PREDICATE_FORALL > (forall VARIABLE_LIST SUPER_PREDICATE )    (P = 1.0000)

FUNCTION_COMPARISON > TWO_ARG_COMPARISON    (P = 0.8880)

FUNCTION_COMPARISON > MULTIPLE_ARGS_EQUAL_COMPARISON    (P = 0.1120)

TWO_ARG_COMPARISON > ( BINARY_COMP COMPARISON_ARG COMPARISON_ARG )    (P = 1.0000)

BINARY_COMP > <=    (P = 0.2000)

BINARY_COMP > <    (P = 0.2000)

BINARY_COMP > =    (P = 0.2000)

BINARY_COMP > >=    (P = 0.2000)

BINARY_COMP > >    (P = 0.2000)

COMPARISON_ARG > FUNCTION_EVAL    (P = 0.5983)

COMPARISON_ARG > COMPARISON_ARG_NUMBER_VALUE    (P = 0.4017)

FUNCTION_EVAL > FUNCTION_BUILDING_SIZE    (P = 0.0753)

FUNCTION_EVAL > FUNCTION_DISTANCE    (P = 0.6774)

FUNCTION_EVAL > FUNCTION_DISTANCE_SIDE_3    (P = 0.0968)

FUNCTION_EVAL > FUNCTION_DISTANCE_SIDE_4    (P = 0.0645)

FUNCTION_EVAL > FUNCTION_X_POSITION    (P = 0.0860)

FUNCTION_BUILDING_SIZE > (building_size PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_OR_FUNCTION_TERM > OBJECT_NAME    (P = 0.5000)

PREDICATE_OR_FUNCTION_TERM > VARIABLE    (P = 0.5000)

OBJECT_NAME > AGENT    (P = 0.0500)

OBJECT_NAME > BED    (P = 0.0500)

OBJECT_NAME > DESK    (P = 0.0500)

OBJECT_NAME > DOOR    (P = 0.0500)

OBJECT_NAME > FLOOR    (P = 0.0500)

OBJECT_NAME > MAIN_LIGHT_SWITCH    (P = 0.0500)

OBJECT_NAME > MIRROR    (P = 0.0500)

OBJECT_NAME > ROOM_CENTER    (P = 0.0500)

OBJECT_NAME > RUG    (P = 0.0500)

OBJECT_NAME > SIDE_TABLE    (P = 0.0500)

OBJECT_NAME > BOTTOM_DRAWER    (P = 0.0500)

OBJECT_NAME > BOTTOM_SHELF    (P = 0.0500)

OBJECT_NAME > EAST_SLIDING_DOOR    (P = 0.0500)

OBJECT_NAME > EAST_WALL    (P = 0.0500)

OBJECT_NAME > NORTH_WALL    (P = 0.0500)

OBJECT_NAME > SOUTH_WALL    (P = 0.0500)

OBJECT_NAME > TOP_DRAWER    (P = 0.0500)

OBJECT_NAME > TOP_SHELF    (P = 0.0500)

OBJECT_NAME > WEST_SLIDING_DOOR    (P = 0.0500)

OBJECT_NAME > WEST_WALL    (P = 0.0500)

FUNCTION_DISTANCE > (distance PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

FUNCTION_DISTANCE_SIDE_3 > (distance_side PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_SIDE_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_OR_FUNCTION_SIDE_TERM > SIDE    (P = 0.5000)

PREDICATE_OR_FUNCTION_SIDE_TERM > SIDE_VARIABLE    (P = 0.5000)

FUNCTION_DISTANCE_SIDE_4 > (distance_side PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_SIDE_TERM PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_SIDE_TERM )    (P = 1.0000)

FUNCTION_X_POSITION > (x_position PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

COMPARISON_ARG_NUMBER_VALUE > NUMBER_PATTERN    (P = 1.0000)

NUMBER_PATTERN > /-?\d*\.?\d+/    (P = 1.0000)

MULTIPLE_ARGS_EQUAL_COMPARISON > (= [ COMPARISON_ARG ]+ )    (P = 1.0000)

PREDICATE > PREDICATE_ABOVE    (P = 0.0112)

PREDICATE > PREDICATE_ADJACENT    (P = 0.0595)

PREDICATE > PREDICATE_ADJACENT_SIDE_3    (P = 0.0165)

PREDICATE > PREDICATE_ADJACENT_SIDE_4    (P = 0.0093)

PREDICATE > PREDICATE_AGENT_CROUCHES    (P = 0.0093)

PREDICATE > PREDICATE_AGENT_HOLDS    (P = 0.2241)

PREDICATE > PREDICATE_BETWEEN    (P = 0.0126)

PREDICATE > PREDICATE_BROKEN    (P = 0.0093)

PREDICATE > PREDICATE_EQUAL_X_POSITION    (P = 0.0093)

PREDICATE > PREDICATE_EQUAL_Z_POSITION    (P = 0.0112)

PREDICATE > PREDICATE_FACES    (P = 0.0119)

PREDICATE > PREDICATE_GAME_OVER    (P = 0.0106)

PREDICATE > PREDICATE_GAME_START    (P = 0.0099)

PREDICATE > PREDICATE_IN    (P = 0.0879)

PREDICATE > PREDICATE_IN_MOTION    (P = 0.2161)

PREDICATE > PREDICATE_IS_SETUP_OBJECT    (P = 0.0165)

PREDICATE > PREDICATE_OBJECT_ORIENTATION    (P = 0.0172)

PREDICATE > PREDICATE_ON    (P = 0.1190)

PREDICATE > PREDICATE_OPEN    (P = 0.0099)

PREDICATE > PREDICATE_OPPOSITE    (P = 0.0106)

PREDICATE > PREDICATE_RUG_COLOR_UNDER    (P = 0.0152)

PREDICATE > PREDICATE_SAME_COLOR    (P = 0.0231)

PREDICATE > PREDICATE_SAME_OBJECT    (P = 0.0126)

PREDICATE > PREDICATE_SAME_TYPE    (P = 0.0172)

PREDICATE > PREDICATE_TOGGLED_ON    (P = 0.0106)

PREDICATE > PREDICATE_TOUCH    (P = 0.0397)

PREDICATE_ABOVE > (above PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_ADJACENT > (adjacent PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_ADJACENT_SIDE_3 > (adjacent_side PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_SIDE_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_ADJACENT_SIDE_4 > (adjacent_side PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_SIDE_TERM PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_SIDE_TERM )    (P = 1.0000)

PREDICATE_AGENT_CROUCHES > (agent_crouches EMPTY_CLOSURE )    (P = 1.0000)

PREDICATE_AGENT_HOLDS > (agent_holds PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_BETWEEN > (between PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_BROKEN > (broken PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_EQUAL_X_POSITION > (equal_x_position PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_EQUAL_Z_POSITION > (equal_z_position PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_FACES > (faces PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_GAME_OVER > (game_over EMPTY_CLOSURE )    (P = 1.0000)

PREDICATE_GAME_START > (game_start EMPTY_CLOSURE )    (P = 1.0000)

PREDICATE_IN > (in PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_IN_MOTION > (in_motion PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_IS_SETUP_OBJECT > (is_setup_object PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_OBJECT_ORIENTATION > (object_orientation PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_ORIENTATION_TERM )    (P = 1.0000)

PREDICATE_OR_FUNCTION_ORIENTATION_TERM > ORIENTATION    (P = 0.5000)

PREDICATE_OR_FUNCTION_ORIENTATION_TERM > ORIENTATION_VARIABLE    (P = 0.5000)

PREDICATE_ON > (on PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_OPEN > (open PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_OPPOSITE > (opposite PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_RUG_COLOR_UNDER > (rug_color_under PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_COLOR_TERM )    (P = 1.0000)

PREDICATE_OR_FUNCTION_COLOR_TERM > COLOR    (P = 0.5000)

PREDICATE_OR_FUNCTION_COLOR_TERM > COLOR_VARIABLE    (P = 0.5000)

PREDICATE_SAME_COLOR > (same_color PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_COLOR_TERM )    (P = 0.6809)

PREDICATE_SAME_COLOR > (same_color PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 0.3191)

PREDICATE_SAME_OBJECT > (same_object PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_SAME_TYPE > (same_type PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TYPE_TERM )    (P = 1.0000)

PREDICATE_OR_FUNCTION_TYPE_TERM > OBJECT_TYPE    (P = 0.5000)

PREDICATE_OR_FUNCTION_TYPE_TERM > VARIABLE    (P = 0.5000)

PREDICATE_TOGGLED_ON > (toggled_on PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

PREDICATE_TOUCH > (touch PREDICATE_OR_FUNCTION_TERM PREDICATE_OR_FUNCTION_TERM )    (P = 1.0000)

SETUP_GAME_OPTIONAL > (game-optional SUPER_PREDICATE )    (P = 1.0000)

CONSTRAINTS_DEF > (:constraints PREFERENCES )    (P = 1.0000)

PREFERENCES > (and [ PREF_DEF ]+ )    (P = 1.0000)

PREF_DEF > PREFERENCE    (P = 0.7092)

PREF_DEF > PREF_FORALL    (P = 0.2908)

PREFERENCE > (preference PREFERENCE_NAME PREF_BODY )    (P = 1.0000)

PREFERENCE_NAME > NAME    (P = 1.0000)

PREF_BODY > PREF_BODY_EXISTS    (P = 0.8496)

PREF_BODY > THEN    (P = 0.0973)

PREF_BODY > AT_END    (P = 0.0531)

PREF_BODY_EXISTS > (exists VARIABLE_LIST THEN )    (P = 0.7843)

PREF_BODY_EXISTS > (exists VARIABLE_LIST AT_END )    (P = 0.2157)

THEN > (then [ SEQ_FUNC ]+ )    (P = 1.0000)

SEQ_FUNC > ONCE    (P = 0.6089)

SEQ_FUNC > ONCE_MEASURE    (P = 0.0242)

SEQ_FUNC > HOLD    (P = 0.2793)

SEQ_FUNC > WHILE_HOLD    (P = 0.0875)

ONCE > (once  SUPER_PREDICATE )    (P = 1.0000)

ONCE_MEASURE > (once-measure SUPER_PREDICATE FUNCTION_EVAL )    (P = 1.0000)

HOLD > (hold SUPER_PREDICATE )    (P = 1.0000)

WHILE_HOLD > (hold-while SUPER_PREDICATE [ SUPER_PREDICATE ]+ )    (P = 1.0000)

AT_END > (at-end SUPER_PREDICATE )    (P = 1.0000)

PREF_FORALL > (forall VARIABLE_LIST PREF_FORALL_PREFS )    (P = 1.0000)

PREF_FORALL_PREFS > (and [ PREFERENCE ]+ )    (P = 1.0000)

TERMINAL_DEF > (:terminal TERMINAL )    (P = 1.0000)

TERMINAL > TERMINAL_AND    (P = 0.1040)

TERMINAL > TERMINAL_OR    (P = 0.2000)

TERMINAL > TERMINAL_NOT    (P = 0.0960)

TERMINAL > TERMINAL_COMP    (P = 0.6000)

TERMINAL_AND > (and [ TERMINAL ]+ )    (P = 1.0000)

TERMINAL_OR > (or [ TERMINAL ]+ )    (P = 1.0000)

TERMINAL_NOT > (not TERMINAL )    (P = 1.0000)

TERMINAL_COMP > TERMINAL_TIME_COMP    (P = 0.1818)

TERMINAL_COMP > TERMINAL_SCORE_COMP    (P = 0.2222)

TERMINAL_COMP > TERMINAL_PREF_COUNT_COMP    (P = 0.5960)

TERMINAL_TIME_COMP > ( BINARY_COMP TOTAL_TIME TIME_NUMBER_VALUE )    (P = 1.0000)

TOTAL_TIME > (total-time)    (P = 1.0000)

TIME_NUMBER_VALUE > NUMBER_PATTERN    (P = 1.0000)

TERMINAL_SCORE_COMP > ( BINARY_COMP TOTAL_SCORE SCORE_NUMBER_VALUE )    (P = 1.0000)

TOTAL_SCORE > (total-score)    (P = 1.0000)

SCORE_NUMBER_VALUE > NUMBER_PATTERN    (P = 1.0000)

TERMINAL_PREF_COUNT_COMP > ( BINARY_COMP SCORING_EXPR_OR_NUMBER PREF_COUNT_NUMBER_VALUE )    (P = 1.0000)

SCORING_EXPR_OR_NUMBER > SCORING_EXPR    (P = 0.7263)

SCORING_EXPR_OR_NUMBER > SCORING_NUMBER_VALUE    (P = 0.2737)

SCORING_EXPR > SCORING_EXTERNAL_MAXIMIZE    (P = 0.0404)

SCORING_EXPR > SCORING_EXTERNAL_MINIMIZE    (P = 0.0187)

SCORING_EXPR > SCORING_MULTI_EXPR    (P = 0.3390)

SCORING_EXPR > SCORING_BINARY_EXPR    (P = 0.0202)

SCORING_EXPR > SCORING_NEG_EXPR    (P = 0.0404)

SCORING_EXPR > PREFERENCE_EVAL    (P = 0.4992)

SCORING_EXPR > SCORING_COMPARISON    (P = 0.0420)

SCORING_EXTERNAL_MAXIMIZE > (external-forall-maximize SCORING_EXPR )    (P = 1.0000)

SCORING_EXTERNAL_MINIMIZE > (external-forall-minimize SCORING_EXPR )    (P = 1.0000)

SCORING_MULTI_EXPR > ( MULTI_OP [ SCORING_EXPR_OR_NUMBER ]+ )    (P = 1.0000)

MULTI_OP > +    (P = 0.5000)

MULTI_OP > *    (P = 0.5000)

SCORING_BINARY_EXPR > ( BINARY_OP SCORING_EXPR_OR_NUMBER SCORING_EXPR_OR_NUMBER )    (P = 1.0000)

BINARY_OP > -    (P = 0.5000)

BINARY_OP > /    (P = 0.5000)

SCORING_NEG_EXPR > (- SCORING_EXPR_OR_NUMBER )    (P = 1.0000)

PREFERENCE_EVAL > COUNT    (P = 0.4305)

PREFERENCE_EVAL > COUNT_OVERLAPPING    (P = 0.0331)

PREFERENCE_EVAL > COUNT_ONCE    (P = 0.0795)

PREFERENCE_EVAL > COUNT_ONCE_PER_OBJECTS    (P = 0.2185)

PREFERENCE_EVAL > COUNT_LONGEST    (P = 0.0265)

PREFERENCE_EVAL > COUNT_SHORTEST    (P = 0.0265)

PREFERENCE_EVAL > COUNT_TOTAL    (P = 0.0265)

PREFERENCE_EVAL > COUNT_INCREASING_MEASURE    (P = 0.0265)

PREFERENCE_EVAL > COUNT_UNIQUE_POSITIONS    (P = 0.0287)

PREFERENCE_EVAL > COUNT_SAME_POSITIONS    (P = 0.0287)

PREFERENCE_EVAL > COUNT_ONCE_PER_EXTERNAL_OBJECTS    (P = 0.0464)

PREFERENCE_EVAL > COUNT_MEASURE    (P = 0.0287)

COUNT > (count PREF_NAME_AND_TYPES )    (P = 1.0000)

PREF_NAME_AND_TYPES > PREFERENCE_NAME [ PREF_OBJECT_TYPE ]*    (P = 1.0000)

PREF_OBJECT_TYPE > : COLOR    (P = 0.2821)

PREF_OBJECT_TYPE > : OBJECT_NAME    (P = 0.0821)

PREF_OBJECT_TYPE > : OBJECT_TYPE    (P = 0.6359)

COUNT_OVERLAPPING > (count-overlapping PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_ONCE > (count-once PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_ONCE_PER_OBJECTS > (count-once-per-objects PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_LONGEST > (count-longest PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_SHORTEST > (count-shortest PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_TOTAL > (count-total PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_INCREASING_MEASURE > (count-increasing-measure PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_UNIQUE_POSITIONS > (count-unique-positions PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_SAME_POSITIONS > (count-same-positions PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_ONCE_PER_EXTERNAL_OBJECTS > (count-once-per-external-objects PREF_NAME_AND_TYPES )    (P = 1.0000)

COUNT_MEASURE > (count-measure PREF_NAME_AND_TYPES )    (P = 1.0000)

SCORING_COMPARISON > SCORING_COMP    (P = 0.6923)

SCORING_COMPARISON > SCORING_EQUALS_COMP    (P = 0.3077)

SCORING_COMP > ( BINARY_COMP SCORING_EXPR_OR_NUMBER SCORING_EXPR_OR_NUMBER )    (P = 1.0000)

SCORING_EQUALS_COMP > (= [ SCORING_EXPR_OR_NUMBER ]+ )    (P = 1.0000)

SCORING_NUMBER_VALUE > NUMBER_PATTERN    (P = 1.0000)

PREF_COUNT_NUMBER_VALUE > NUMBER_PATTERN    (P = 1.0000)

SCORING_DEF > (:scoring SCORING )    (P = 1.0000)

SCORING > SCORING_EXPR    (P = 1.0000)

## Token rule expansions

NAME > triangle_block_green    (P = 0.0063)

NAME > bed    (P = 0.0068)

NAME > west_wall    (P = 0.0063)

NAME > cube_block    (P = 0.0263)

NAME > sliding_door    (P = 0.0074)

NAME > north_wall    (P = 0.0063)

NAME > book    (P = 0.0121)

NAME > hexagonal_bin    (P = 0.0711)

NAME > cylindrical_block    (P = 0.0121)

NAME > tall_rectangular_block_blue    (P = 0.0063)

NAME > flat_block_yellow    (P = 0.0063)

NAME > drawer    (P = 0.0090)

NAME > desktop    (P = 0.0095)

NAME > flat_block_tan    (P = 0.0063)

NAME > shelf    (P = 0.0116)

NAME > tall_cylindrical_block    (P = 0.0100)

NAME > bridge_block    (P = 0.0121)

NAME > west_sliding_door    (P = 0.0063)

NAME > key_chain    (P = 0.0090)

NAME > tall_rectangular_block    (P = 0.0063)

NAME > tall_cylindrical_block_tan    (P = 0.0063)

NAME > top_shelf    (P = 0.0063)

NAME > desk    (P = 0.0063)

NAME > pyramid_block_red    (P = 0.0074)

NAME > dodgeball    (P = 0.0632)

NAME > room_center    (P = 0.0063)

NAME > chair    (P = 0.0158)

NAME > cd    (P = 0.0095)

NAME > bridge_block_green    (P = 0.0063)

NAME > triangular_ramp    (P = 0.0116)

NAME > game_object    (P = 0.0237)

NAME > ramp    (P = 0.0063)

NAME > dodgeball_blue    (P = 0.0095)

NAME > flat_block    (P = 0.0090)

NAME > teddy_bear    (P = 0.0137)

NAME > pyramid_block    (P = 0.0132)

NAME > cube_block_blue    (P = 0.0105)

NAME > wall    (P = 0.0153)

NAME > south_wall    (P = 0.0063)

NAME > golfball_orange    (P = 0.0063)

NAME > doggie_bed    (P = 0.0200)

NAME > pyramid_block_yellow    (P = 0.0074)

NAME > triangle_block_tan    (P = 0.0063)

NAME > pen    (P = 0.0074)

NAME > bridge_block_tan    (P = 0.0063)

NAME > mug    (P = 0.0079)

NAME > cube_block_yellow    (P = 0.0105)

NAME > flat_block_gray    (P = 0.0063)

NAME > door    (P = 0.0063)

NAME > cylindrical_block_blue    (P = 0.0063)

NAME > pyramid_block_blue    (P = 0.0079)

NAME > golfball_white    (P = 0.0063)

NAME > bottom_shelf    (P = 0.0063)

NAME > tall_rectangular_block_green    (P = 0.0063)

NAME > shelf_desk    (P = 0.0074)

NAME > top_drawer    (P = 0.0068)

NAME > tall_cylindrical_block_green    (P = 0.0063)

NAME > main_light_switch    (P = 0.0074)

NAME > laptop    (P = 0.0100)

NAME > triangle_block_blue    (P = 0.0063)

NAME > pillow    (P = 0.0137)

NAME > dodgeball_red    (P = 0.0084)

NAME > triangular_ramp_green    (P = 0.0068)

NAME > east_wall    (P = 0.0063)

NAME > beachball    (P = 0.0184)

NAME > golfball    (P = 0.0195)

NAME > watch    (P = 0.0074)

NAME > mirror    (P = 0.0063)

NAME > side_table    (P = 0.0068)

NAME > lamp    (P = 0.0074)

NAME > pencil    (P = 0.0074)

NAME > blinds    (P = 0.0074)

NAME > floor    (P = 0.0074)

NAME > bridge_block_pink    (P = 0.0063)

NAME > cellphone    (P = 0.0095)

NAME > rug    (P = 0.0068)

NAME > alarm_clock    (P = 0.0105)

NAME > golfball_green    (P = 0.0079)

NAME > cylindrical_block_green    (P = 0.0063)

NAME > ball    (P = 0.0274)

NAME > cylindrical_block_tan    (P = 0.0063)

NAME > basketball    (P = 0.0158)

NAME > credit_card    (P = 0.0068)

NAME > cube_block_tan    (P = 0.0068)

NAME > tall_rectangular_block_tan    (P = 0.0063)

NAME > building    (P = 0.0169)

NAME > bottom_drawer    (P = 0.0063)

NAME > tall_cylindrical_block_yellow    (P = 0.0063)

NAME > curved_wooden_ramp    (P = 0.0153)

NAME > triangular_ramp_tan    (P = 0.0063)

NAME > triangle_block    (P = 0.0079)

NAME > block    (P = 0.0211)

NAME > poster    (P = 0.0063)

NAME > east_sliding_door    (P = 0.0063)

NAME > dodgeball_pink    (P = 0.0105)

BINARY_COMP > <=    (P = 0.1733)

BINARY_COMP > <    (P = 0.1733)

BINARY_COMP > =    (P = 0.2933)

BINARY_COMP > >=    (P = 0.2000)

BINARY_COMP > >    (P = 0.1600)

NUMBER_PATTERN > 0    (P = 0.0118)

NUMBER_PATTERN > 1    (P = 0.0749)

NUMBER_PATTERN > 2    (P = 0.0461)

NUMBER_PATTERN > 3    (P = 0.0548)

NUMBER_PATTERN > 4    (P = 0.0403)

NUMBER_PATTERN > 5    (P = 0.0432)

NUMBER_PATTERN > 6    (P = 0.0432)

NUMBER_PATTERN > 7    (P = 0.0375)

NUMBER_PATTERN > 8    (P = 0.0403)

NUMBER_PATTERN > 9    (P = 0.0346)

NUMBER_PATTERN > 10    (P = 0.0548)

NUMBER_PATTERN > 0.5    (P = 0.0128)

NUMBER_PATTERN > 0.6    (P = 0.0118)

NUMBER_PATTERN > 0.7    (P = 0.0128)

NUMBER_PATTERN > 0.2    (P = 0.0118)

NUMBER_PATTERN > 0.1    (P = 0.0118)

NUMBER_PATTERN > 0.3    (P = 0.0118)

NUMBER_PATTERN > 0.8    (P = 0.0118)

NUMBER_PATTERN > 0.4    (P = 0.0118)

NUMBER_PATTERN > 0.9    (P = 0.0118)

NUMBER_PATTERN > 330    (P = 0.0870)

NUMBER_PATTERN > 300    (P = 0.0024)

NUMBER_PATTERN > 270    (P = 0.0870)

NUMBER_PATTERN > 240    (P = 0.0870)

NUMBER_PATTERN > 210    (P = 0.0870)

NUMBER_PATTERN > 180    (P = 0.1014)

NUMBER_PATTERN > 150    (P = 0.0870)

NUMBER_PATTERN > 120    (P = 0.0870)

NUMBER_PATTERN > 90    (P = 0.0118)

NUMBER_PATTERN > 60    (P = 0.0118)

NUMBER_PATTERN > 30    (P = 0.0158)

NUMBER_PATTERN > 20    (P = 0.0346)

NUMBER_PATTERN > 40    (P = 0.0138)

NUMBER_PATTERN > 50    (P = 0.0138)

NUMBER_PATTERN > 70    (P = 0.0118)

NUMBER_PATTERN > -50    (P = 0.0118)

NUMBER_PATTERN > 80    (P = 0.0118)

NUMBER_PATTERN > -40    (P = 0.0118)

NUMBER_PATTERN > -30    (P = 0.0118)

NUMBER_PATTERN > 100    (P = 0.0158)

NUMBER_PATTERN > -20    (P = 0.0118)

NUMBER_PATTERN > -10    (P = 0.0138)

NUMBER_PATTERN > -9    (P = 0.0118)

NUMBER_PATTERN > -8    (P = 0.0118)

NUMBER_PATTERN > -7    (P = 0.0118)

NUMBER_PATTERN > -6    (P = 0.0118)

NUMBER_PATTERN > -5    (P = 0.0148)

NUMBER_PATTERN > -4    (P = 0.0118)

NUMBER_PATTERN > -3    (P = 0.0148)

NUMBER_PATTERN > -2    (P = 0.0118)

NUMBER_PATTERN > -1    (P = 0.0118)

NUMBER_PATTERN > 11    (P = 0.0346)

NUMBER_PATTERN > 12    (P = 0.0375)

NUMBER_PATTERN > 13    (P = 0.0346)

NUMBER_PATTERN > 14    (P = 0.0346)

NUMBER_PATTERN > 15    (P = 0.0375)

NUMBER_PATTERN > 16    (P = 0.0375)

NUMBER_PATTERN > 17    (P = 0.0346)

NUMBER_PATTERN > 18    (P = 0.0375)

NUMBER_PATTERN > 19    (P = 0.0346)

NUMBER_PATTERN > 21    (P = 0.0346)

NUMBER_PATTERN > 22    (P = 0.0346)

NUMBER_PATTERN > 23    (P = 0.0346)

NUMBER_PATTERN > 24    (P = 0.0346)

NUMBER_PATTERN > 25    (P = 0.0346)

NUMBER_PATTERN > -25    (P = 0.0118)

NUMBER_PATTERN > -24    (P = 0.0118)

NUMBER_PATTERN > -23    (P = 0.0118)

NUMBER_PATTERN > -22    (P = 0.0118)

NUMBER_PATTERN > -21    (P = 0.0118)

NUMBER_PATTERN > -19    (P = 0.0118)

NUMBER_PATTERN > -18    (P = 0.0118)

NUMBER_PATTERN > -17    (P = 0.0118)

NUMBER_PATTERN > -16    (P = 0.0118)

NUMBER_PATTERN > -15    (P = 0.0118)

NUMBER_PATTERN > -14    (P = 0.0118)

NUMBER_PATTERN > -13    (P = 0.0118)

NUMBER_PATTERN > -12    (P = 0.0118)

NUMBER_PATTERN > -11    (P = 0.0118)

TOTAL_TIME > (total-time)    (P = 1.0000)

TOTAL_SCORE > (total-score)    (P = 1.0000)

MULTI_OP > +    (P = 0.3000)

MULTI_OP > *    (P = 0.7000)

BINARY_OP > -    (P = 0.4800)

BINARY_OP > /    (P = 0.5200)
\end{lstlisting}

==> human_evaluations_mann_whitney.tex <==
% Throwing a copy of everything here before I start shifting the narrative to be mixed-model centric.

\subsection*{Human evaluations}
\label{sec:human-evals}
To systematically and extrinsically evaluate our model, we performed human evaluations using a second set of human participants ($n = 100$; see \autoref{fig:methods-human-evals-interface} for the evaluation interface and \nameref{methods:human-evals} for details).
% We tasked these participants with evaluating games for human likeness, fun, creativity, and other factors, for a total of seven measures. 
Evaluated games belonged to one of three different categories mentioned above:
\texttt{real} participant-created games from our behavioral experiment, or \texttt{matched} or \texttt{unmatched} model-generated games (see \autoref{fig:model-overview} for category definitions; games in \autoref{fig:model-comparison} and \autoref{fig:novel-texts} were included; see \nameref{methods:human-evals} for details).
%\texttt{real} games created by participants in our first experiment, \texttt{matched} games (one corresponding to and occupying the same niche as each \texttt{real} game), and novel \texttt{unmatched} games (games in \autoref{fig:model-comparison} and \autoref{fig:novel-texts} were included; see \nameref{methods:human-evals} for details).
% Rather than ask participants to interpret our domain-specific language, we back-translate games to structured natural language descriptions using the GPT-4 language model \cite{OpenAI2023GPT-4} (see \nameref{methods:human-evals} for details).
Participants evaluated three games in each category above (without knowing their categories) in a randomized order and provided Likert scale ratings on each game for seven measures, including human likeness, fun, and creativity. Our final dataset includes 892 participant-game evaluations, each with a rating for all seven measures.

\input{tables/human_evals/human_eval_mann_whitney_table}

\autoref{tab:mann-whitney} summarizes the quantitative responses from our human evaluations. 
We begin with a simple statistical comparison of the ratings of the games in the different categories using the nonparametric Mann-Whitney $U$-test \cite{MannWhitney1947} (and see \nameref{methods:human-evals} for additional details).
Participants respond similarly to the \texttt{real} and \texttt{matched} games, with no statistically significant differences in the average response scores across all seven attributes.
On the other hand, the \texttt{unmatched} games differ on a number of attributes. Compared to both \texttt{real} and \texttt{matched} games, participants judge them to be less easily understood, less fun to play and watch, and less human-like.
One potential explanation for the apparent similarity between \texttt{matched} and \texttt{real} games is that the former simply replicate the latter in form and function. 
We examined this question and found that \texttt{matched} and \texttt{real} games have substantial functional differences (see summary in \autoref{fig:real-matched-comparison}, details in \cref{sec:appendix-matched-real-similarity}, and methodological details in \nameref{methods:similarity}).

To further analyze these differences and the extent to which they are mediated by our fitness measure, we performed a mixed-effects regression analysis whose results are summarized in \autoref{tab:mixed-models}.
We fit independent models using each of the seven attributes we asked our human evaluators to judge as the dependent variables. 
We include fixed effects for the fitness score and membership in the \texttt{real} and \texttt{matched} groups (treating the \texttt{unmatched} group as a baseline), and random effects for the participants and individual games (see \nameref{methods:human-evals} and Supplementary \cref{tab:supplementary-mixed-models} for full details).
We find that our fitness function captures many of the evaluated attributes: higher fitness predicts higher ratings of understandability, fun to play, and human likeness ($\beta_{\text{fit}} > 0$); conversely, higher fitness also predicts lower ratings of helpfulness, difficulty, and creativity ($\beta_{\text{fit}} < 0$). 
Our positive findings are promising: they indicate that our fitness function, learned to maximize human likeness in a symbolic program space, also captures intuitive human notions of understandability and fun. 
Conversely, we view the negative relations as evidence of some degree of mode-seeking: our fitness measure likely assigns the highest scores to the games most representative of the dataset at large.
These modal games are plausibly neither particularly creative nor difficult, which means that participants might find also them less helpful for learning the details of the environment. 
Finally, differences in attribute ratings persist between groups even accounting for any mediating effects of fitness scores (see \cref{sec:appendix-mixed-effect-analyses} for details)

We also performed ablations of key model components corresponding to the cognitive capacities we found our participants recruited.
To ablate \textit{physical common sense}, we remove from our fitness function the two features that estimate the feasibility of a game's preferences by leveraging our database of participant-environment interactions. Analogously, we ablate the intuitive \textit{coherence} we observe in human goals by removing the features that capture the coordination of gameplay elements between different sections. Ablating \textit{compositionality} is more difficult, as our programmatic representation is inherently compositional. We do so by removing the crossover mutation operator used to generate new samples during MAP-Elites, which most explicitly leverages the compositional structure of games. 
In all cases, model performance degrades substantially, either in sample fitness scores or in goal plausibility as estimated using our database of participant-environment interactions (see \cref{sec:appendix-ablations} for further details).

==> old_notes.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.35\columnwidth]{figures/overview.png}
%     \caption{Dummy overview figure}
%     \label{fig:overview}
% \end{figure}

% Concretely, our contributions are:
% \begin{enumerate}
%     \item We present a set of hundreds of game features and a process for training an energy model that leverages them in order to differentiate between high-quality (i.e. ``human-like'') and low-quality games described in our DSL
%     \item We describe a set of ``behavioral characteristics'' (features along which we expect generated games to be diverse) and the method for adapting a quality diversity algorithm to our problem
%     \item We demonstrate that our approach is capable of producing samples that \TODO[approach human quality in a variety of automated metrics]
% \end{enumerate}

% \section{Related Work}
% \subsection{Automatic Game Design}
% Within the field of procedural content generation (PCG), a variety of approaches have been explored for the generation of novel game rulesets. Rulesets are typically represented as programs in a domain-specific language (DSL), and optimization methods are used to search through the space of programs for ``high-quality'' games. Past efforts have largely focused on board games \cite{pell1992metagame, browne2010evolutionary} and video games \cite{togelius2008experiment, smith2010ludocore, khalifa2017general}, and have made use of heuristic evaluation, evolutionary optimization, and tree search. While the reliable generation of human-quality games remains elusive, these approaches have yielded at least some notable success: the commercially-available game \texttt{YAVALATH} was designed by an automated system \cite{browne2011yavalath}. Our work continues the branch of game generation through evolutionary optimization, though we focus on a new domain (human-like embodied games) and learn a fitness function from a dataset of samples rather than relying fully an expert knowledge.

% \subsection{Goal Generation in RL}
% Recent advances in reinforcement learning have allowed agents to dynamically set goals for themselves either as part of training or during an episode \cite{florensa2018automatic}. Most approaches define goals as particular regions of state space \cite{florensa2018automatic} or as particular world states expressed as conjunctions of logical or semantic primitives \cite{team2021open, team2023human, akakzia2020grounding}. Recent work has made use of large language models, either to express goals explicitly in natural language \cite{huang2023inner, shah2023lm} or to generate programs which encode the goal \cite{liang2023code, kwon2022reward, wang2023voyager}. Our work represents goals not as instantaneously-evaluable functions over single states, but rather as temporal sequences of states, aligning more closely with work in the planning domain \cite{silver2022pddl}. We also emphasize the plausibility of generated goals with respect to a human dataset as part of an effort to better understand the process through which humans produce novel goals.

% \subsection{Program Synthesis via Quality Diversity}
%  Our work also broadly falls under the umbrella of genetic programming, with an emphasis on diversity of programs and a measure of quality relative to an existing dataset rather than an external evaluator. The issue of diversity in genetic programming is well-studied \cite{burke2004diversity, ekart2002maintaining, burks2015efficient}, and there have been some efforts to apply explicit quality-diversity methods \cite{boisvert2021quality, dolson2019exploring}, including in the context of games \cite{khalifa2018talakat}. 

% \TODO

% Things we should make sure to mention:
% \begin{itemize}
%     \item The Cameron Brown paper
%     \item Approaches to goal generation in RL -- e.g. Cedric's review paper, and some of the other ones I cited in the original paper? Some of the newer language and LLM-based ones? 
%     \item Other approaches that use programs in some way -- e.g. VOYAGER (\url{https://arxiv.org/abs/2305.16291}), or Text2Reward (\url{https://text-to-reward.github.io/}).
%     \item Other papers doing program induction/generation using MAP-Elites or similar approaches?
%     \item Open-ended goal generation, e.g. XLand (\url{https://arxiv.org/abs/2107.12808}) and XLand 2 (\url{https://arxiv.org/abs/2301.07608})
% \end{itemize}

% While the energy model defined above gives a sense of the ``quality'' of a given game, simple optimization of this objective would explore only a tiny fraction of the space of human-like games. We use \texttt{MAP-Elites} \cite{mouret2015illuminating}, a popular evolutionary quality-diversity algorithm, to illuminate a larger swath of the search space by defining a set of \textit{behavioral characteristics} across which games are optimized independently in a multi-dimensional ``archive.'' Following prior work on using \texttt{MAP-Elites} for procedural content generation \cite{charity2020mech}, we define a set binary behavioral characteristics that each indicate the presence of particular archetypal game components (i.e. a ball, or the use of the \texttt{adjacent} predicate)  -- the algorithm attempts to find a high-quality game for each possible combination of values under the behavioral characteristics. We use \textcolor{red}{10} such features for a total archive size of \textcolor{red}{1024}.

% Initial samples for the algorithm are generated by sampling from the MAP estimate of our grammar PCFG (see \autoref{sec:objectve-function}). That is, the algorithm does \textit{not} start with corruptions of existing games, as we use to produce the negatives mentioned above. %\textit{maximum a posteriori} estimate of our grammar learned from the set of human games. 
% At each step, a game is chosen uniformly from among the exemplars in each cell of the archive and mutated by either \textbf{regrowing} a random node and its children in its syntax tree, \textbf{inserting \& deleting} the child of a node with multiple potential children, \textbf{crossing over} with the syntax tree of another randomly-selected game, and a few \textbf{custom mutation operators}.
% These include resampling a preference by replacing the variables it quantifies, or the initial or terminal conditions of its temporal modals. 
% We also use operators that sample or resample the optional game sections (setup and terminal conditions).
% The resulting game is evaluated to determine both its fitness and its assignment under each of the behavioral characteristics (i.e. cell in the archive) -- if its fitness is greater than that of the current exemplar, the new game replaces it. \textbf{\textcolor{red}{Full details of the algorithm are available in the Appendix.}}

% \subsection{Sampling Games}

% In order to generate novel games, we use \textit{maximum a posteriori} (MAP) estimation. In particular, for each rule in our grammar, we fit a distribution using the occurrence rates in our dataset of human generated games and a prior of \TODO[what prior do we use?]. This allows us to produce samples in two ways -- either by iteratively sampling from the distribution, starting at the root of our grammar, or by ``regrowing'' an existing game. To regrow a game, we select a node from its tree representation uniformly at random, delete its children, and then re-sample new children iteratively from the MAP estimate.

% \subsection{Energy Model}

% We choose as our primary evaluation function an energy model -- a single-layer neural network without an activation function that maps from a game's set of features to a real-valued energy score. The energy model is trained to distinguish between our dataset of human-generated games (referred to as ``positives'' in this context) and a set of ``negatives'' produced by the simple grammatical sampling procedure described above. Specifically, for each of 98 positives in our dataset (split into 62 training games, 16 validation games, and 20 held-out test games), we sample 1024 negatives. During training, we sample a random batch of negatives for each positive and optimize the weights to minimize energy softmin loss -- i.e. to assign low energy scores to the positive and high energy scores to each of its regrown negatives. We perform 5-fold cross validation and use the validation results on the test set to select our training hyperparameters. Once the hyperparameters have been selected, we use them to train one final model on the entire dataset (all 98 games and their associated negatives), which becomes the energy model used in our experiments. The optimization process is described in detail in Algorithm~\ref{alg:energy-model-training}, and hyperparameters are available in the Appendix.

% \subsection{Search Procedure}

% Our aim is to produce a set of generated games that both resemble human games (i.e. are given low scores by our energy mode) and cover a wide range of semantic possibilities. To that end, we make use a \textit{quality diversity} algorithm -- namely, MAP-Elites \cite{mouret2015illuminating}. MAP-Elites works by defining a set of ``behavioral characteristics,'' or phenotype features across which samples should be diverse. The behavioral characteristics are typically discretized into a number of bins in order to form a multi-dimensional archive, with any given sample occupying a specific cell in the archive depending on its evaluation under the behavioral characteristics. At each step algorithm operates by randomly selecting a member of the current archive, applying a mutation operator, and evaluating the new sample under the fitness function and each of the behavioral characteristics. The behavioral characteristics are used to determine which cell the new sample would occupy in the archive. If the cell is unoccupied, then the new sample is added. Otherwise, the new sample's fitness is compared to the current occupant's fitness -- the sample with the greater fitness is kept and the other is discarded. This process is described in detail in Algorithm~\ref{alg:map-elites}.

% \subsection{Mutation}
% At each step of the algorithm, after an elite has been selected for modification, we randomly sample and apply a mutation operator from the following list.
% {\flushleft \textbf{Regrowth:}} We randomly select a node and re-sample its children from the MAP estimate

% {\flushleft \textbf{Insertion \& Deletion:}} We randomly select a node from the game which can have a variable number of children (e.g. an \texttt{and} operator), weighted such that nodes with fewer children are more likely to be selected, and sample an additional child from the MAP estimate to be inserted. Afterwards, we perform a ``context-fixing'' pass on the game, ensuring that any previously-unseen variables referred to in the new child are properly defined. Finally, we independently sample a node with multiple children, delete one them, and perform the context-fixing pass again (removing definitions to any variables that are no longer used). 

% {\flushleft \textbf{Crossover:}} \TODO[Describe how we do crossover (e.g. with typing based on the node expansion rules]

% {\flushleft \textbf{Bespoke operators:}} \TODO[Describe the various bespoke operators we have in brief, and what they do (with more detail in an Appendix?)]

% \subsection{Behavioral Characteristics}

% For our behavioral characteristics, we take inspiration from \texttt{MechElites} \cite{charity2020mech}, which used the MAP-Elites algorithm to produce game levels that required the use of specific game mechanics in order to solve. The \texttt{MechElites} approach uses a set of binary behavioral characteristics that each indicate whether a particular game mechanic is used in a given level. We adapt this to our domain by selecting behavioral characteristics that each indicate whether a game either contains a particular predicate or a variable of a particular type. Our set of 8 behavioral characteristics is as follows, leading to a total archive size of 256. \TODO[Talk about other BC selections?]
% \begin{itemize}
%     \item Does the game contain either the \texttt{agent\_holds} or \texttt{in\_motion} predicate?
%     \item Does the game contain the \texttt{in} predicate?
%     \item Does the game contain the \texttt{on} or \texttt{touch} predicate?
%     \item Does the game contain the \texttt{adjacent} or \texttt{between} predicate?
%     \item Does the game refer to either a \texttt{block} or a \texttt{building}?
%     \item Does the game refer either a piece of \texttt{furniture} or a \texttt{room feature}?
%     \item Does the game refer to either a \texttt{small object} or a \texttt{large object}?
%     \item Does the game refer to either a \texttt{ball} or a \texttt{receptacle}?
% \end{itemize}

% \section{Model and Algorithm}

% \subsection{Search Procedure}
% In order to generate samples, we use the MAP-Elites algorithm. MAP-Elites is an evolutionary quality-diversity algorithm that attempts to produce a set of problem solutions that are both high fitness and distinct from one another. In its simplest form, MAP-Elites functions as follows:

% To begin, the algorithm works by specifying a set of ``behavioral characteristics,'' or feature dimensions across which solutions should be diverse, as well as a fitness function that determines a candidate solution's quality. Each behavioral characteristic is defined by some mapping from candidate solutions to a binary or scalar value, and the outputs of each behavioral characteristic are then discretized into two or more mutually-exclusive ``cells.'' The discretized behavioral characteristics are then combined to form a multi-dimensional grid of cells referred to as the ``archive.'' By construction, every candidate solution occupies exactly one cell in the archive based on its feature values under the behavioral characteristics.

% The algorithm then proceeds by generating a collection of initial solutions. Each candidate solution is evaluated both in terms of fitness and under the behavioral characteristics in order to determine which cell of the archive it occupies. If more than one candidate solution would occupy the same cell, then only the highest-fitness solution is kept and the rest are discarded. The occupant of a given cell is referred to as an ``elite.''

% After the initial solutions have been generated, each step of the algorithm consists of selecting a candidate solution from among the elites currently in the archive and performing some sort of mutation operator on it. The modified solution is then evaluated in terms of fitness and the behavioral characteristics. If the modified solution would occupy a previously-unoccupied cell, then it is added to the archive and becomes that cell's elite. If the modified solution would occupy an \textit{occupied} cell, then its fitness is compared to the cell's current elite. If the modified solution's fitness is higher, then it replaces that cell's elite. Otherwise, it is discarded. This process continues until the algorithm is terminated.

% Because candidate solutions are only directly compared to other solutions in the same cell, MAP-Elites is able to achieve a diverse array of high-fitness solutions by building on so-called `stepping stone` solutions that represent initial ventures into unexplored regions of the search space without those solutions being forced out of the population by existing high-fitness individuals. 

% \subsection{Fitness Function}
% \textcolor{red}{[TODO: Explain the Energy Model]}

% \subsection{Behavioral Characteristics}
% The performance of MAP-Elites is highly-dependent on the choice of behavioral characteristics. The behavioral characteristics determine the kind of variation maintained by the archive, and in addition the total size of the archive scales linearly with the number of cells per behavioral characteristic and exponentially with the number of characteristics themselves.

% For this work, we choose as our behavioral characteristics a subset of the compositional features described in (CITATION), as well as proxy measures of a game's complexity. Specifically, we use:
% \textcolor{red}{[TODO: describe specific BCs used]}

% \subsection{Initial Samples}
% In order to encourage a diversity of samples in the archive, we generate our collection of initial samples using the following procedure. \textcolor{red}{[TODO: explain initial sampling protocol]}

% \subsection{Mutation Operators}
% At each step, an elite is selected and then mutated in order to form a new candidate solution. We define a set of mutation operators, described below, and randomly select an operator to apply at each step.

% \subsubsection{Regrowth}
% To perform this mutation operator, we select a random node in the tree representation of the game, delete it and its children, and then resample the subtree. This resampling is done using the probabilistic context-free grammar (PCFG) learned from our dataset of human games.

% \subsubsection{Insertion}
% To perform this mutation operator, we select a random node in the tree representation of the game which can resolve to a variable number of children under our grammar (for instance, the \texttt{(and)} operator can take two or more children representing the arguments of the conjunction). We then use the PCFG to sample another child and insert it under the selected node. The selection process is weighted by the number of children for each valid node, such that nodes with fewer children are more likely to be selected for insertion. Finally, after inserting the child we perform a ``context-fixing'' step in which we attempt to ensure that any new variables quantified by the insertion step are referred to at least once in the following preference.

% \subsubsection{Deletion}
% The deletion operator closely resembles the insertion operator described above. We use the same process to randomly select a valid node with at least two children, except here we invert the weighting such that nodes with many children are more likely to be selected. We then delete one of the children from the tree and perform context-fixing to remove references to a variable which is no longer quantified as a result of the deletion.

% \subsubsection{Cognitively-Plausible Operators}
% \textcolor{red}{[TODO?]}

% \subsection{Elite Selection Strategies}
% In the basic implementation of MAP-Elites, the process for selecting an elite at each step to mutate is completely random. However, prior work has demonstrated that selection strategies based on the principles of multi-arm bandits are more effective (CITATION). We use the following selection strategies in our experiments:

% \section{Background}
% Inspired by the notion of play as ``learning to create and solve arbitrary challenges,'' \cite{Chu2020} 
% We build on previous work \cite{DavidsonGuerckisLake2022} studying game creation as the capacity to generate playful cognitive goals. 
%we view games as a powerful and flexible way to represent cognitive goals. 
% We represent these cognitive goals as structured programs in a domain-specific language (DSL). 
% This representation has its root in Language of Thought (LoT) approaches, and such program-like encodings have been used in a variety of cognitive science domains \cite{Rule2020}. 
% Similarly, artificial autotelic agents make use of auto-generated goals in order to self-direct their learning and exploration \cite{Colas2020review}, though such approaches typically define goals as particular regions of state space \cite{florensa2018automatic, Campero2020, team2021open} or, more recently, as linguistic descriptions generated by and evaluated with large language models \cite{huang2023inner, Du2023, Colas2023, wang2023voyager}.
% Other approaches, such as GLTL \cite{Littman2017} or reward machines \cite{ToroIcarte2022} allow representing temporally-extended, non-Markovian goals. 
% We borrow from Icarte et al. \cite{ToroIcarte2022} the notion of these goals operating as programs over sequences of states, emitting reward when appropriate, but using a domain-specific language capable of representing human games. 
% Our work also falls broadly in the realm of automatic game design, which has mostly focused on board games \cite{pell1992metagame, browne2010evolutionary} and video games \cite{togelius2008experiment, smith2010ludocore, khalifa2017general}. While reliably producing human-quality and non-trivial games remains an open challenge, evolutionary approaches have yielded at least some success when combined with expert knowledge \cite{browne2011yavalath}. 

% Our DSL has four main components, two of which are mandatory, and two of which are optional \TODO[We probably want to anchor this to a specific example, right? I can update a figure from a previous paper].
% Any game must include gameplay preferences, which specify how a game is to be played. 
% These can be either specifications of temporal conditions, specified in temporal modals that map onto linear temporal logic (LTL, \cite{Manna1992}) formulas, or static conditions that must hold at the end of the game.
% Additionally, a game must include scoring rules, which describe how to count satisfactions of the defined preferences and how to combine them into a final score.
% The optional sections include setup conditions that must be satisfied before gameplay can commence and terminal conditions that specify when a game ends. 
% See \cite{DavidsonGuerckisLake2022} for a longer description of various aspects of the DSL, and \TODO[Appendix ???] for a full specification.
% Inspired by \cite{ToroIcarte2022}, we implement our own reward machine, an interpreter of our DSL, which can parse state-action traces of an agent interacting with an environment and emit rewards as appropriate.
% In the future, the reward machine could allow training RL agents to play games or perform other tasks specified in this DSL, but that is beyond the scope of this work.
% However, we currently use this reward machine as part of the game generation procedure and to filter out potentially invalid games, see \TODO[refer to the appropriate section] for additional details.

% We work with the dataset collected by \cite{DavidsonGuerckisLake2022}, which consists of a mere \textit{98 human games}, manually translated from natural language to this DSL. 
% We next describe how we learn an objective function to quantify 'human-likeness' in this domain, and then outline the search procedure we use to generate novel, human-like games.  

% To search the space of games for new programs that are human-like, we are confronted with numerous challenges.
% While representing the DSL as a probabilistic context-free grammar (PCFG) aids in sampling expressions from it (see \TODO[appendix with the PCFG representation]), the lack of context means that the space of programs representable in the DSL is larger than the space of validly interpretable programs (for instance, a program could refer to a nonexistent variable). 
% Game programs could also be valid, but semantically incoherent: this could be by generating logical contradictions of predicates, or sequences of temporal models that are unsatisfiable. 
% Even when programs do not fail on the logical level, they could lack common sense: for instance, by stipulating that a tower be built by stacking balls, rather than blocks, or that objects be placed on a wall, rather than, say, next to it. 
% With a much larger dataset, perhaps some (or all) of these constraints could be learned end-to-end by a large language model from the textual and reward program descriptions of games. 
% However, we are interested in solutions that do not require internet-scale data, as we are inspired by children, who display the ability to conjure up games to entertain themselves from a young age \CITEHERE[something about kids coming up with games].
% We therefore opt to learn an objective function over an extracted feature representation of games, with features representing various desiderata of games.
% We learn the objective function using a novel conservative, energy-based procedure, using our grammar to generate mild corruptions from our existing human games. 

% For evaluating a program's fitness, we represent it as a feature vector using a custom feature set.
% Extracting a feature vector (as opposed to operating over the textual or syntax-tree representations) allows us to use a simple energy model and include properties that we envisioned would be important for generating novel, human-like game programs.
% This is also a practical choice: we suspected that learning a fitness function end-to-end from a textual representation of the game programs would be impractical with the 98 human games we collected, and experiments using embeddings extracted from pretrained LLMs proved futile.
% \TODO[full feature appendix] offers a comprehensive description of our feature set. 
% Some of our features try to provide additional context to the PCFG game program representations, such as checking if all defined variables are referenced, or if all preferences are used at least once. 
% We use n-gram models over the syntax tree representations to provide a proto-language model, and try to estimate the feasibility of generated predicate expressions by searching for predicate satisfactions in the state-action traces of our human participant interactions. 
% Other features help check for coherence across different program components, such as checking that successive temporal modals operate over shared sets of variables. 
% We also include some features that capture the size of the generated programs: the length and maximal depth in each section, and the number of preferences included. 
% Every feature we extract is either a binary value, a proportion between zero and one, or if it is a floating point value, we normalize it to the unit interval over the dataset of real and regrown games we generate (see next subsection).


% Below, we provide a number of example feature categories and features in each category. 
% \begin{itemize}
%     \setlength{\itemsep}{1em}
%     \item \textbf{Additional context:} we represent our grammar as a probabilistic context-free grammar, but several contextual elements can aid in generating proper programs. These include the proportion of variables defined that were referenced at least once, the proportion of preferences defined that were used at least once, and whether any variable names were defined twice in any context.

%     \item \textbf{N-gram features:} we extract n-gram tokens from an in-order traversal of the syntax tree. We use 5-gram models with stupid backoff \CITEHERE[stupid backoff] with a discount factor of 0.4, and report the mean log score as the feature value, both jointly over the entire game program and separately over the different sections (setup, preferences, terminal conditions, and scoring).

%     \item 
    
%     % \item \textbf{N-gram features:} we perform an in-order traversal of the syntax tree and extract n-grams. Terminals that refer to an object or type are replaced with a category (e.g. \lstinline{dodgeball} is replaced with \lstinline{ball}, or \lstinline{bed} with \lstinline{furniture}), and type nodes are represented by their rule. We compute separate n-gram scores for the entire game and for each section (setup, preferences, terminal conditions, and scoring)independently, 
% \end{itemize}


==> removed_commented_out_bits.tex <==
%% Old results wrapfigure
% \begin{wrapfigure}{r}{0.4 \textwidth}
%     % \vspace{-0.9in}
%     \centering
%     \includegraphics[width=.39 \textwidth]{figures/map_elites_quantitative_reuslts_vertical_top_only.png}
%     \vspace{-0.1in}
%     \caption{MAP-Elites quantitative results.
%     %Our model fills the archive, quickly (within a few hundred generations) finding games in the human fitness range, and gradually increasing the mean archive fitness until it also falls in the human game range.
%     }
%     \label{fig:results-quantitative}
%     % \vspace{-0.65in}
% \end{wrapfigure}




%% Ablations
%%% Common sense
% Many features in our feature set help capture different kinds of common sense, some more semantically and others more programmatically. 
% \autoref{sec:appendix-features} enumerates our entire feature set, and \autoref{sec:appendix-predictive-features} highlights the features that are most predictive of real and regrown games.
% We elaborate briefly on a few features that encapsulate different types of common sense below:
% \begin{easylist}
% @ \texttt{predicate\_found\_in\_data\_prop}: this feature uses a dataset of participant interactions in our environment to approximate predicate-argument feasibility. We enumerate every predicate in a game, ground its variable arguments to their types, and count the proportion of which that occurred at least once in a participant's gameplay. An expression such as ``ball on chair'' would count positively, while an expression like ``chair on wall'' would count negatively.

% @ \texttt{variables\_used\_all}, \texttt{preferences\_used\_all}: these features capture a more programmatic type of common sense. Nothing in the grammar precludes quantifying a variable but never referring to it, or doing the same with an entire gameplay preference---but there is no reason to do so. These features have a value of 1 if all variables or predicates (respectively) are referenced at least once, or 0 if at least one is unused.

% @ \texttt{repeated\_variables\_found}: another type of illogical yet grammatically valid expression is applying a predicate on the same object as both arguments---such as checking ``is the ball in the ball''? or ``is the bed next to the bed?'' This feature captures such failure modes. 

% % Other good candidates: \texttt{predicate\_without\_variables\_or\_agent}, texttt{redundant\_expression\_found}, \texttt{two\_number\_operation\_found}
% \end{easylist}

%%% Creativity
% \begin{easylist}
% @ In very early experiments, we attempted to use 10 different compositional patterns identified in \cite{DavidsonGuerckisLake2022} as the behavioral features. While we found our model was capable of generating high-fitness functions for these features, upon inspection we discovered the samples were all \textit{highly} similar to each other -- we did not achieve meaningful diversity.

% @ Unless we explicitly included the number of preferences a game uses as a behavioral feature, we found almost all games in our archive to include only a single preference. We view this bias toward simplicity as reflecting the fact that our initial proposals are low fitness, and it takes the model substantial work (and many generations) to improve candidates---so absent pressure to include longer samples, the model would only produce short ones. \autoref{fig:fitness-by-n-prefs} confirms this intuition by plotting the fitness across both human and model-generated games by the number of preferences---fitness in single-preference games is significantly higher than all other preference counts\footnote{We limited our model to up to four preferences to cap archive size, and so we exclude four of the 98 human games that have five or more preferences.}
% \end{easylist}

% \subsection{Context-sensitivity}
% For completeness of the discussion with 

% \textbf{Context-sensitivity:}
% \begin{easylist}
%     @ I think we made a brief note that our current model does not tackle this sort of grounding, but we could, e.g. by limiting sampled object type terminals to a relevant subset
% \end{easylist}


% \subsection{Complexity}
% \label{sec:complexity}
% \begin{easylist}
%     @ This should probably be (some of) what's currently in the Creativity section, and discuss the BCs more there. 
%     % @ I think the simplest analysis of what I had to say about complexity went in the creativity section -- I could imagine (1) keeping it there and not discussing complexity separately, (2) changing that header to creativity and complexity, or (3) moving this here and discussing creativity in a different fashion (perhaps relating to some of the analyses Graham is running to demonstrate that our model isn't just spitting out identical copies to the human dataset. 
% \end{easylist}

==> tables/ablations/pref_count_correlation_table.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\begin{adjustbox}{center}
\begin{threeparttable}
\caption{\textbf{Attribute and length correlation summary}  }
\label{tab:pref-count-correlations}
\begin{tabular}{lrrrrrrrrr}
\toprule
\textbf{Measure} & \textit{Understandable} & \textit{Fun to play} & \textit{Fun to watch} & \textit{Helpful} & \textit{Difficult} & \textit{Creative} & \textit{Human-like} & \textit{Preferences} & \textit{Length} \\
 \midrule
\textit{Understandable} & 1.000 & 0.437 & 0.330 & -0.130 & -0.409 & -0.322 & 0.596 & -0.400 & -0.290 \\
\textit{Fun to play} & 0.437 & 1.000 & 0.876 & 0.444 & 0.223 & 0.463 & 0.782 & -0.091 & 0.172 \\
\textit{Fun to watch} & 0.330 & 0.876 & 1.000 & 0.504 & 0.263 & 0.566 & 0.711 & -0.115 & 0.168 \\
\textit{Helpful} & -0.130 & 0.444 & 0.504 & 1.000 & 0.245 & 0.579 & 0.317 & 0.249 & 0.266 \\
\textit{Difficult} & -0.409 & 0.223 & 0.263 & 0.245 & 1.000 & 0.661 & -0.024 & 0.348 & 0.430 \\
\textit{Creative} & -0.322 & 0.463 & 0.566 & 0.579 & 0.661 & 1.000 & 0.224 & 0.313 & 0.512 \\
\textit{Human-like} & 0.596 & 0.782 & 0.711 & 0.317 & -0.024 & 0.224 & 1.000 & -0.258 & 0.008 \\
\textit{Preferences} & -0.400 & -0.091 & -0.115 & 0.249 & 0.348 & 0.313 & -0.258 & 1.000 & 0.732 \\
\textit{Length} & -0.290 & 0.172 & 0.168 & 0.266 & 0.430 & 0.512 & 0.008 & 0.732 & 1.000 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \item \textbf{Length measures correlate positively with creativity and difficulty, but not with understandability or human-likeness.} 
    We compute, for each evaluated game, its mean score in each evaluated attribute.
    We then compute correlation coefficients between these per-game mean scores. 
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}




==> tables/ablations/pref_count_correlation_table_small.tex <==

\begin{table}[!htbp]
\centering
\normalsize
\begin{adjustbox}{center}
\begin{threeparttable}
\caption{\textbf{Attribute and length correlation summary}  }
\label{tab:pref-count-correlations}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{\textit{Number of Preferences}} & \multicolumn{2}{c}{\textit{Program Length}}  \\
\textbf{Measure} & $\rho_{\texttt{prefs}}$ & Significance &  $\rho_{\texttt{length}}$ & Significance \\
 \midrule
\textit{Understandable}     & -0.4   & *** & -0.29 & **  \\
\textit{Fun to play}        & -0.091 & -   & 0.172 & -   \\
\textit{Fun to watch}       & -0.115 & -   & 0.168 & -   \\
\textit{Helpful}            & 0.249  & *   & 0.266 & *   \\
\textit{Difficult}          & 0.348  & *** & 0.43  & *** \\
\textit{Creative}           & 0.313  & **  & 0.512 & *** \\
\textit{Human-like}         & -0.258 & *   & 0.008 & -   \\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \item \textbf{Length measures correlate positively with creativity and difficulty, but not with understandability or human-likeness.} 
    We compute each evaluated game's mean score in each evaluated attribute.
    We then compute (Pearson) correlation coefficients and significance tests on these per-game mean scores. 
    *: $P < 0.05$, **: $P < 0.01$, ***: $P< 0.001$
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}






==> tables/human_evals/marginal_means_summary_with_fitness.tex <==
\begin{table}[!btph]
\centering
\footnotesize
\begin{adjustbox}{center}
\begin{threeparttable}
\caption{\textbf{Mixed model result summary}  }
\label{tab:marginal-means-summary}
% \begin{tabular}{|p{3cm}|rrl|rrl|rrl|}

% VERSION 1: Split by variable, then by beta / Z / P
\begin{tabular}{lcccccccc}

% VERSION 2: Split by beta / Z / P, then by variable
% \begin{tabular}{lcccccc}

\toprule
%% VERSION 1
& \multicolumn{8}{c}{\textbf{Pair Comparison}} \\
& \multicolumn{2}{c}{\texttt{Real} $-$ \texttt{Matched}} & & \multicolumn{2}{c}{\texttt{Real} $-$ \texttt{Unmatched} } & &  \multicolumn{2}{c}{\texttt{Matched} $-$ \texttt{Unatched} } \\
\textbf{Measure} & Diff $\pm SE$ & Significance & & Diff $\pm SE$ & Significance & & Diff $\pm SE$ & Significance \\

%% VERSION 2
% & \multicolumn{3}{c}{\textbf{Coefficient}} & \multicolumn{3}{c}{\textbf{Significance}} \\
% \textbf{Measure} & \texttt{Fitness} & $\mathbbm{1}[\texttt{Matched}]$ & $\mathbbm{1}[\texttt{Real}]$ & \texttt{Fitness} & $\mathbbm{1}[\texttt{Matched}]$ & $\mathbbm{1}[\texttt{Real}]$ \\


\midrule

%% VERSION 1
\textit{Understandable} $\uparrow$ & $0.626 \pm 0.305$ & - & & $1.151 \pm 0.285$ & *** & & $0.525 \pm 0.297$  & - \\ 
   \textit{Fun to play} $\uparrow$ & $0.430 \pm 0.273$ & - & & $1.059 \pm 0.263$ & *** & & $0.629 \pm 0.274$ & - \\  
  \textit{Fun to watch} $\uparrow$ & $0.271 \pm 0.264$ & - & & $0.912 \pm 0.257$ & ** & & $0.641 \pm 0.266$ &  *  \\  
  \textit{Helpful}\textsuperscript{\textdagger} $\uparrow$  & $-0.117 \pm 0.167$ & - & & $0.232 \pm 0.161$ & - & & $0.349 \pm 0.170$ & - \\ 
  \textit{Difficult} ${\downarrow \atop \uparrow }$ & $-0.613 \pm 0.355$ & - & & $-0.250 \pm 0.338$ & - & & $0.363 \pm 0.353$ & - \\ 
  \textit{Creative} $\uparrow$  & $-0.113 \pm 0.310$ & - & & $0.438 \pm 0.298$ & - & & $0.551 \pm 0.310$ & - \\ 
  \textit{Human-like} $\uparrow$ & $0.609 \pm 0.265$ &  - & & $1.446 \pm 0.258$ & ***  & & $0.837 \pm 0.268$ &  **  \\ 

%% VERSION 2
% \textit{Understandable} & 0.846 & 0.525 & 1.151 & *** & - & *** \\

% Understandability & 0.846 & 5.625 & $P < \num{1e-5}^{ *** }$ & 0.525 & 1.766 & $P = 0.078$ & 1.151 & 4.036 & $P < \num{1e-3}^{ *** }$ \\ 
%   Fun to play & 0.396 & 2.936 & $P = 0.003^{**}$ & 0.629 & 2.298 & $P = 0.022^*$ & 1.059 & 4.021 & $P < \num{1e-3}^{ *** }$ \\ 
%   Fun to watch & 0.191 & 1.469 & $P = 0.142$ & 0.641 & 2.414 & $P = 0.016^*$ & 0.912 & 3.547 & $P < \num{1e-3}^{ *** }$ \\ 
%   Helpful for interacting in the environment & -0.189 & -2.163 & $P = 0.031^*$ & 0.349 & 2.048 & $P = 0.041^*$ & 0.232 & 1.441 & $P = 0.15$ \\ 
%   Appropriately difficult & -0.588 & -3.443 & $P < \num{1e-3}^{ *** }$ & 0.363 & 1.029 & $P = 0.304$ & -0.250 & -0.740 & $P = 0.46$ \\ 
%   Creatively designed & -0.486 & -3.191 & $P = 0.001^{**}$ & 0.551 & 1.776 & $P = 0.076$ & 0.438 & 1.467 & $P = 0.142$ \\ 
%   Human-likeness & 0.570 & 4.316 & $P < \num{1e-3}^{ *** }$ & 0.837 & 3.128 & $P = 0.002^{**}$ & 1.446 & 5.597 & $P < \num{1e-5}^{ *** }$ \\ 

\bottomrule
\end{tabular}
\begin{tablenotes}
    \item \textbf{Evaluators don't distinguish between participant-created \texttt{real} and \texttt{matched} model games, but do distinguish \texttt{unmatched} games from \texttt{real} (and marginally from  \texttt{matched} ones).} 
    Participants responded to seven Likert questions on a 5-point scale, one for each attribute in the first column (see \nameref{methods:human-evals}). 
    We found fairly low inter-rater agreement (see \cref{sec:appendix-human-evals-analysis}), and so we center our analysis on our fitted mixed-effects models (see \nameref{methods:human-evals}). 
    We use the method of estimated (least-squares) marginal means to compare between the three game groups, accounting for the effect of fitness scores and the random effects fitted to particular games and human evaluators. \\
    We report two-sided significance tests adjusted using the Tukey method to control for the multiple difference tests within each attribute, as implemented in the \texttt{emmeans} package.
    See Supplementary \autoref{tab:supplementary-marginal-means} for test statistics and P-values. 
    *: $P < 0.05$, **: $P < 0.01$, ***: $P< 0.001$ \\
    \textdagger: The full measure description is ``Helpful for interacting with the simulated environment.'' \\
    In most measures, higher scores are better, indicated by the $\uparrow$, other than \textit{Difficult}  ${\downarrow \atop \uparrow }$, in which 3 means ``appropriately difficult'', and scores below and above indicate too easy and too hard respectively.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}

==> tables/model/game_comparison_table.tex <==
\begin{table}[!htbp]
\caption{\textbf{Comparison between real games and corresponding MAP-Elites generations, with programs}}
\label{tab:comparison-with-dsl} 
\begin{adjustbox}{center}
\begin{tabular}{|p{1.5cm}|p{\gamecolumnwidth}|p{\gamecolumnwidth}|p{\gamecolumnwidth}|}
\toprule
\textbf{Game ID} & \textbf{Participant Game \#0} (fitness 36.583) & \textbf{Participant Game \#14} (fitness 36.491) & \textbf{Participant Game \#31} (fitness 37.338) \\
\midrule
\textbf{Participant Game Text (GPT-4 back-translated)} & { \small  
\textbf{Setup:} place a hexagonal bin near a triangular ramp and make sure they stay in place throughout the game. 

\textbf{Gameplay:} hold a ball and throw it so that it touches the triangular ramp and then lands inside the hexagonal bin. 

\textbf{Terminal:} the game ends when the hexagonal bin, which must start standing upright, is no longer upright without being touched or held by you. 

\textbf{Scoring:} you earn 1 point for each time you successfully throw a ball that touches the ramp and lands in the bin.  } & { \small  

\textbf{Gameplay:} stack a flat block on a bridge block, then place a tall cylindrical block on the flat block, followed by a cube block on the tall cylindrical block, and finally a pyramid block on the cube block. 

\textbf{Scoring:} you get 10 points for each different set of blocks you have successfully stacked in this order by the end of the game.  } & { \small  

\textbf{Gameplay:} throw a ball so that it touches a wall and then either catch it or touch it 

\textbf{Scoring:} you get 1 point for each time you successfully throw the ball, it touches a wall, and you are either holding it again or touching it after its flight  } \\
\textbf{Participant Game DSL Program} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game 6172feb1665491d1efbce164-0) (:domain medium)
(:setup
  (exists (?h - hexagonal_bin ?r - triangular_ramp)
    (game-conserved (near ?h ?r)
)))
(:constraints (and
    (preference throwToRampToBin
      (exists (?b - ball ?r - triangular_ramp ?h - hexagonal_bin)
        (then
          (once (agent_holds ?b))
          (hold-while (and (not (agent_holds ?b)) (in_motion ?b)) (touch ?b ?r))
          (once (and (not (in_motion ?b)) (in ?h ?b)))
   )))
    (preference binKnockedOver
      (exists (?h - hexagonal_bin)
        (then
          (once (object_orientation ?h upright))
          (hold (and (not (touch agent ?h)) (not (agent_holds ?h))))
          (once (not (object_orientation ?h upright)))
)))))
(:terminal (>= (count-once binKnockedOver) 1))
(:scoring (count throwToRampToBin))
) \end{lstlisting} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game 613e4bf960ca68f8de00e5e7-17) (:domain medium)
(:constraints
  (and
    (preference castleBuilt
      (exists (?b - bridge_block ?f - flat_block ?t - tall_cylindrical_block ?c - cube_block ?p - pyramid_block)
        (at-end
          (and
            (on ?b ?f)
            (on ?f ?t)
            (on ?t ?c)
            (on ?c ?p)
))))))
(:scoring
  (* 10 (count-once-per-objects castleBuilt))
)) \end{lstlisting} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game 614fb15adc48d3f9ffcadd41-39) (:domain many)
(:constraints
  (and
    (preference ballThrownToWallToAgent
      (exists (?b - ball ?w - wall)
        (then
          (once (agent_holds ?b))
          (hold-while (and (not (agent_holds ?b)) (in_motion ?b)) (touch ?w ?b))
          (once (or (agent_holds ?b) (touch agent ?b)))
)))))
(:scoring
  (count ballThrownToWallToAgent)
)) \end{lstlisting} \\
\midrule
\textbf{Sample} & \textbf{Model Sample} (fitness 37.162) & \textbf{Model Sample} (fitness 36.994) & \textbf{Model Sample} (fitness 37.324) \\
\midrule
\textbf{Model Game Text (GPT-4 back-translated)} & { \small  

\textbf{Setup:} put a hexagonal bin near the rug and ensure it remains there for the duration of the game. 

\textbf{Gameplay:} throw dodgeballs aiming to land them inside the hexagonal bin or on a doggie bed. 

\textbf{Scoring:} you earn points for each dodgeball that comes to rest either inside the hexagonal bin or on the doggie bed, with your final score being the sum of these successful throws.  } & { \small  

\textbf{Gameplay:} stack three blocks on top of a tall rectangular block, with two of the stacked blocks being the same type as the tall rectangular block. 

\textbf{Scoring:} your score is 1.4 times the number of such stacks you have at the end of the game.  } & { \small  

\textbf{Gameplay:} throw dodgeballs so that they land and come to rest on the top shelf 

\textbf{Terminal:} the game ends after 30 seconds 

\textbf{Scoring:} you get 1 point for each dodgeball that is resting on the top shelf at the end of the game  } \\
\textbf{Model Game DSL Program} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game evo-8180-66-0) (:domain medium)
(:setup
  (exists (?v0 - hexagonal_bin)
    (game-conserved
      (near rug ?v0)
)))
(:constraints
  (and
    (preference preference0
      (exists (?v0 - hexagonal_bin ?v1 - dodgeball)
        (then
          (once (agent_holds ?v1))
          (hold (and (not (agent_holds ?v1)) (in_motion ?v1)))
          (once (and (not (in_motion ?v1)) (in ?v0 ?v1)))
   )))
    (preference preference1
      (exists (?v0 - dodgeball ?v1 - doggie_bed)
        (then
          (once (agent_holds ?v0))
          (hold (and (not (agent_holds ?v0)) (in_motion ?v0)))
          (once (and (not (in_motion ?v0)) (on ?v1 ?v0)))
)))))
(:scoring
  (+ (count preference1) (count preference0))
)) \end{lstlisting} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game evo-8176-22-0) (:domain many)
(:constraints
  (and
    (preference preference0
      (exists (?v0 - block ?v1 - block ?v2 - tall_rectangular_block ?v3 - block)
        (at-end
          (and
            (on ?v2 ?v0)
            (on ?v2 ?v1)
            (on ?v2 ?v3)
            (same_type ?v0 ?v2)
            (same_type ?v1 ?v2)
))))))
(:scoring
  (+ (* 0.4 (count preference0))
    (count preference0)
))) \end{lstlisting} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game evo-8175-229-0) (:domain few)
(:constraints
  (and
    (preference preference0
      (exists (?v0 - dodgeball)
        (then
          (once (agent_holds ?v0))
          (hold (and (not (agent_holds ?v0)) (in_motion ?v0)))
          (once (and (not (in_motion ?v0)) (on top_shelf ?v0)))
)))))
(:terminal
  (>= (total-time) 30)
)
(:scoring
  (count preference0)
)) \end{lstlisting} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}




==> tables/model/game_novel_sample_table.tex <==
\begin{table}[!htbp]
\caption{\textbf{Novel MAP-Elites generations, with programs}}
\label{tab:novel-with-dsl}
\begin{adjustbox}{center}
\begin{tabular}{|p{1.5cm}|p{\gamecolumnwidth}|p{\gamecolumnwidth}|p{\gamecolumnwidth}|}
\toprule
\textbf{Game ID} & \textbf{Model Sample} (fitness 36.066) & \textbf{Model Sample} (fitness 36.446) & \textbf{Model Sample} (fitness 37.096) \\
\midrule
\textbf{Model Game Text (GPT-4 back-translated)} & { \small  \textbf{Setup:} place a hexagonal bin near the north wall and make sure it stays there throughout the game.

 \textbf{Gameplay:} throw golfballs aiming to have them stop on and inside the hexagonal bin, and stack blocks so that each has three cube blocks on top, with one cube block being the same type as the block it's on.

 \textbf{Scoring:} you score points based on the number of correctly stacked blocks minus four times the number of golfballs that stop on and inside the hexagonal bin.  } & { \small  \textbf{Gameplay:} pick up and put down green triangle blocks, throw dodgeballs onto the desk, and throw basketballs onto a hexagonal bin.

 \textbf{Scoring:} you get 1 point for each time you pick up and put down a green triangle block, 1 point for each dodgeball that stops on the desk, and 1 point for each basketball that stops on a hexagonal bin.  } & { \small  \textbf{Gameplay:} throw dodgeballs so that they land inside a hexagonal bin or on a doggie bed

 \textbf{Scoring:} you get 1 point for each dodgeball that stops moving inside the hexagonal bin and 1 point for each dodgeball that stops moving on the doggie bed  } \\
\textbf{Model Game DSL Program} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game evo-8172-48-1) (:domain many)
(:setup
  (exists (?v0 - hexagonal_bin)
    (game-conserved
      (near north_wall ?v0)
)))
(:constraints
  (and
    (preference preference0
      (exists (?v0 - hexagonal_bin ?v1 - golfball)
        (then
          (once (agent_holds ?v1))
          (hold (and (not (agent_holds ?v1)) (in_motion ?v1)))
          (once (and (on ?v0 ?v1) (not (in_motion ?v1)) (in ?v0 ?v1)))
   )))
    (preference preference1
      (exists (?v0 - cube_block ?v2 - cube_block ?v3 - block ?v4 - cube_block)
        (at-end
          (and
            (on ?v3 ?v0)
            (on ?v3 ?v2)
            (on ?v3 ?v4)
            (same_type ?v4 ?v3)
))))))
(:scoring
  (+ (* -4 (count preference0))
    (count preference1)
))) \end{lstlisting} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game evo-8142-307-1) (:domain many)
(:constraints
  (and
    (preference preference0
      (exists (?v0 - triangle_block_green)
        (then
          (once (agent_holds ?v0))
          (hold (not (agent_holds ?v0)))
          (hold (agent_holds ?v0))
          (once (not (in_motion ?v0)))
   )))
    (preference preference1
      (exists (?v1 - dodgeball)
        (then
          (once (agent_holds ?v1))
          (hold (and (not (agent_holds ?v1)) (in_motion ?v1)))
          (once (and (not (in_motion ?v1)) (on desk ?v1)))
   )))
    (preference preference2
      (exists (?v0 - hexagonal_bin ?v1 - basketball)
        (then
          (once (agent_holds ?v1))
          (hold (and (not (agent_holds ?v1)) (in_motion ?v1)))
          (once (and (not (in_motion ?v1)) (on ?v0 ?v1)))
)))))
(:scoring
  (+ (count preference0) (count preference2) (count preference1))
)) \end{lstlisting} & \begin{lstlisting}[aboveskip=-0.4 \baselineskip,belowskip=-0.8 \baselineskip]
(define (game evo-8149-344-0) (:domain medium)
(:constraints
  (and
    (preference preference0
      (exists (?v0 - hexagonal_bin ?v1 - dodgeball)
        (then
          (once (agent_holds ?v1))
          (hold (and (not (agent_holds ?v1)) (in_motion ?v1)))
          (once (and (not (in_motion ?v1)) (in ?v0 ?v1)))
   )))
    (preference preference1
      (exists (?v0 - dodgeball ?v1 - doggie_bed)
        (then
          (once (agent_holds ?v0))
          (hold (and (not (agent_holds ?v0)) (in_motion ?v0)))
          (once (and (not (in_motion ?v0)) (on ?v1 ?v0)))
)))))
(:scoring
  (+ (count preference1) (count preference0))
)) \end{lstlisting} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}




==> tables/model/text_only_comparison_table.tex <==
% \begin{wraptable}{r}{2.2 \textcolumnwidth}
%     \vspace{-0.75in}
%     \caption{\textbf{MAP-Elites generates simple human-like goals.} Each pair of games in a row has the same set of MAP-Elites behavioral characteristics (\autoref{sec:search})} 
%     \begin{adjustbox}{center}
%     \begin{tabular}{|p{\textcolumnwidth}|p{\textcolumnwidth}|}
%     \toprule
%     \textbf{Real Games} & \textbf{MAP-Elites Samples} \\
%     \midrule
%     { \tiny Throw dodgeballs into the bin. You get a point for each made throw. } &  { \tiny Throw beachballs into the bin. The game ends after you've made 22 throws or 5 throws with different beachballs. You get a point for each made throw. } \\ \midrule
%     { \tiny Build a `castle' by grabbing a bridge block, a flat block, a tall cylindrical block, a cube block, and a pyramid block, and stack them on top of each other in that order } &  { \tiny Make buildings by grabbing a green bridge block, and placing any block and a pyramid block on it. The game ends once you make 12 such structures, and you get a point for each. } \\ \midrule
% { \tiny Set up the game by placing the dodgeball near the center of the room. To play the game, make a building on top of the doggie bed, without objects touching the floor or a wall. You get a point for each object in the building. } &  { \tiny Set up the game by placing the hexagonal bin very close to the east wall. To play, put blue cube blocks on shelves adjacent to the west wall, and place orange objects closer to the rug than to the door. The game ends after you've placed 23 blue cube blocks or 20 different orange objects, and you get a point for each blue cube block placed. } \\ 
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     \label{tab:comparison-texts}
%     \vspace{-0.2in}
% \end{wraptable}

\begin{table}[!htbp]
    % \vspace{-0.75in}
\caption{\textbf{MAP-Elites generates simple human-like games.} Each pair of games in a column has the same set of MAP-Elites behavioral characteristics. Parentheses: the fitness score assigned by the model to each game.} 
\label{tab:comparison-texts}
\begin{adjustbox}{center}
\begin{tabular}{|p{\textcolumnwidth}|p{\textcolumnwidth}|p{\textcolumnwidth}|}
\toprule
\textbf{Participant Game \#0} (36.583) & \textbf{Participant Game \#14} (36.491) & \textbf{Participant Game \#31} (37.338) \\
\midrule
{ \small  
\textbf{Setup:} place a hexagonal bin near a triangular ramp and make sure they stay in place throughout the game. 

\textbf{Gameplay:} hold a ball and throw it so that it touches the triangular ramp and then lands inside the hexagonal bin. 

\textbf{Terminal:} the game ends when the hexagonal bin, which must start standing upright, is no longer upright without being touched or held by you. 

\textbf{Scoring:} you earn 1 point for each time you successfully throw a ball that touches the ramp and lands in the bin.  } & { \small  

\textbf{Gameplay:} stack a flat block on a bridge block, then place a tall cylindrical block on the flat block, followed by a cube block on the tall cylindrical block, and finally a pyramid block on the cube block. 

\textbf{Scoring:} you get 10 points for each different set of blocks you have successfully stacked in this order by the end of the game.  } & { \small  

\textbf{Gameplay:} throw a ball so that it touches a wall and then either catch it or touch it 

\textbf{Scoring:} you get 1 point for each time you successfully throw the ball, it touches a wall, and you are either holding it again or touching it after its flight  } \\
\\
\midrule
\textbf{Model Sample} (37.162) & \textbf{Model Sample} (36.994) & \textbf{Model Sample} (37.324) \\
\midrule
{ \small  

\textbf{Setup:} put a hexagonal bin near the rug and ensure it remains there for the duration of the game. 

\textbf{Gameplay:} throw dodgeballs aiming to land them inside the hexagonal bin or on a doggie bed. 

\textbf{Scoring:} you earn points for each dodgeball that comes to rest either inside the hexagonal bin or on the doggie bed, with your final score being the sum of these successful throws.  } & { \small  

\textbf{Gameplay:} stack three blocks on top of a tall rectangular block, with two of the stacked blocks being the same type as the tall rectangular block. 

\textbf{Scoring:} your score is 1.4 times the number of such stacks you have at the end of the game.  } & { \small  

\textbf{Gameplay:} throw dodgeballs so that they land and come to rest on the top shelf 

\textbf{Terminal:} the game ends after 30 seconds 

\textbf{Scoring:} you get 1 point for each dodgeball that is resting on the top shelf at the end of the game  } \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-0.2in}
\end{table}

==> tables/model/text_only_novel_sample_table.tex <==
% \begin{wraptable}{r}{1.1 \gamecolumnwidth}
\begin{table}[!htpb]
% \vspace{-0.8in}
\caption{\textbf{MAP-Elites generates interesting, novel goals.} Each of the three games below has high fitness and fills a cell in the MAP-Elites archive with no corresponding human game in our dataset. Each sample's fitness score is in parentheses.}
\label{tab:novel-texts}
\begin{adjustbox}{center}
\begin{tabular}{|p{\textcolumnwidth}|p{\textcolumnwidth}|p{\textcolumnwidth}|}
\toprule
\textbf{Novel Model Sample} (36.066) & \textbf{Novel Model Sample} (36.446) & \textbf{Novel Model Sample} (37.096) \\
\midrule
{ \small  \textbf{Setup:} place a hexagonal bin near the north wall and make sure it stays there throughout the game.

 \textbf{Gameplay:} throw golfballs aiming to have them stop on and inside the hexagonal bin, and stack blocks so that each has three cube blocks on top, with one cube block being the same type as the block it's on.

 \textbf{Scoring:} you score points based on the number of correctly stacked blocks minus four times the number of golfballs that stop on and inside the hexagonal bin.  } & { \small  \textbf{Gameplay:} pick up and put down green triangle blocks, throw dodgeballs onto the desk, and throw basketballs onto a hexagonal bin.

 \textbf{Scoring:} you get 1 point for each time you pick up and put down a green triangle block, 1 point for each dodgeball that stops on the desk, and 1 point for each basketball that stops on a hexagonal bin.  } & { \small  \textbf{Gameplay:} throw dodgeballs so that they land inside a hexagonal bin or on a doggie bed

 \textbf{Scoring:} you get 1 point for each dodgeball that stops moving inside the hexagonal bin and 1 point for each dodgeball that stops moving on the doggie bed  } \\
\bottomrule
\end{tabular}
\end{adjustbox}

    % \vspace{-0.2in}
\end{table}
